The Differential Structure of an Orbifold

We prove that the underlying set of an orbifold equipped with the ring of smooth real-valued functions completely determines the orbifold atlas. Consequently, we obtain an essentially injective functor from orbifolds to differential spaces.

==> metamatter.tex <==
%Note that this file uses the ifthen and hyperref LaTeX packages.

%Diagram options

\input xy
\xyoption{all}

%Space between paragraphs:

\setlength{\parskip}{.5\baselineskip}

% "End of Example" symbol - thanks to Yael Karshon for this (modified):
\def\eoe{\unskip\ \hglue0mm\hfill$\lozenge$\smallskip\goodbreak}

% -- To Make Parenthetical Titles Bold

\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
}
\makeatother


%Notations - \mathbb

\renewcommand{\AA}{{\mathbb{A}}} %adeles or affine
\newcommand{\BB}{{\mathbb{B}}}  %unit ball
\newcommand{\CC}{{\mathbb{C}}}  %complex numbers
\newcommand{\DD}{{\mathbb{D}}}  %unit disk
\newcommand{\EE}{{\mathbb{E}}}  %euclidean space
\newcommand{\FF}{{\mathbb{F}}}  %field
\newcommand{\HH}{{\mathbb{H}}}  %quaternion numbers
\newcommand{\NN}{{\mathbb{N}}}  %natural numbers
\newcommand{\PP}{{\mathbb{P}}}  %projective
\newcommand{\QQ}{{\mathbb{Q}}}  %rational numbers
\newcommand{\RR}{{\mathbb{R}}}  %real numbers or cartesian space
\renewcommand{\SS}{{\mathbb{S}}} %sphere
\newcommand{\TT}{{\mathbb{T}}}  %torus
\newcommand{\XX}{{\mathbb{X}}}  %dunno...
\newcommand{\ZZ}{{\mathbb{Z}}}  %integers

%Notations - \operatorname

\newcommand{\Ad}{{\operatorname{Ad}}}  %adjoint operator
\newcommand{\ad}{{\operatorname{ad}}}  %infinitesimal adjoint operator
\newcommand{\Alt}{{\operatorname{Alt}}}  %alternating functor
\newcommand{\Aut}{{\operatorname{Aut}}}  %automorphisms
\newcommand{\curv}{{\operatorname{curv}}}   %curvature
\newcommand{\D}{{\operatorname{D}}}  %differential operator
\newcommand{\Der}{{\operatorname{Der}}}  %derivations functor
\newcommand{\Diff}{{\operatorname{Diff}}}  %diffeomorphisms
\newcommand{\End}{{\operatorname{End}}}  %endomorphisms
\newcommand{\ev}{{\operatorname{ev}}}   %evaluation map
\renewcommand{\Gauge}{{\operatorname{Gauge}}} %Gauge groupoid
\newcommand{\Gr}{{\operatorname{Gr}}}  %Gromov-Witten invariant
\newcommand{\Grc}{{\operatorname{Gr}_0}} %connected Gromov-Witten invariant
\newcommand{\Ham}{{\operatorname{Ham}}} %hamiltonian diffeomorphisms
\newcommand{\ham}{{\operatorname{ham}}} %hamiltonian vector fields
\newcommand{\Hol}{{\operatorname{Hol}}} %holonomy group
\newcommand{\Hom}{{\operatorname{Hom}}} %Hom
\newcommand{\id}{{\operatorname{id}}}  %identity
\newcommand{\im}{{\operatorname{im}}}  %image
\newcommand{\inter}{{\operatorname{int}}} %interior
\newcommand{\Mat}{{\operatorname{Mat}}} %matrices
\newcommand{\PD}{{\operatorname{PD}}}  %Poincare dual
\newcommand{\pr}{{\operatorname{pr}}} %projection
\newcommand{\Rep}{{\operatorname{Rep}}} %representations
\newcommand{\rk}{{\operatorname{rk}}}  %rank
\newcommand{\sgn}{{\operatorname{sgn}}}  %signum
\newcommand{\Span}{{\operatorname{span}}}  %span
\newcommand{\Stab}{{\operatorname{Stab}}} %stabiliser
\newcommand{\supp}{{\operatorname{supp}}}  %support
\newcommand{\Sym}{{\operatorname{Sym}}}  %symmetric functor
\newcommand{\Symp}{{\operatorname{Symp}}} %symplectomorphisms
\newcommand{\Vect}{{\operatorname{vect}}}  %vector fields

%Notations - Lie

\newcommand{\G}{{\operatorname{G}}} %generic Lie group
\newcommand{\g}{{\mathfrak{g}}} %generic Lie algebra
\newcommand{\GL}{{\operatorname{GL}}}  %general linear
\newcommand{\lie}[1]{{\mathfrak{\lowercase{#1}}}} %Lie algebra of a Lie group
\renewcommand{\O}{{\operatorname{O}}} %orthogonal
\newcommand{\SL}{{\operatorname{SL}}}  %special linear
\newcommand{\SO}{{\operatorname{SO}}}  %special orthogonal
\newcommand{\Sp}{{\operatorname{Sp}}} %symplectic linear
\newcommand{\SU}{{\operatorname{SU}}}  %special unitary
\newcommand{\U}{{\operatorname{U}}}  %unitary

%Notations - Other

\newcommand{\Ck}{{C^k}} %k-differentiable
\newcommand{\CIN}{{C^\infty}}   %infinitely differentiable
\newcommand{\del}{\partial}  % del
\newcommand{\delbar}{\overline{\partial}}  % del-bar
\newcommand{\eps}{\varepsilon}  %var epsilon
\newcommand{\ftimes}[2]{{\lrsubscripts{\times}{#1}{#2}}} %fibre product
\newcommand{\toto}{{~\rightrightarrows~}} %groupoid double arrow
\newcommand{\hook}{{\lrcorner\,}} %hook or interior multiplication
\newcommand{\limit}[1]{{\underset{#1}{\lim}}} %limit
\newcommand{\mar}{{\mathfrak{m}}}  %Marshall ideal
\newcommand{\mtrx}[2]{{\left[\begin{array}{#1}#2 \end{array}\right]}} %matrix
\newcommand{\pois}[2]{{\{#1,#2\}}}  %Poisson bracket
\newcommand{\red}[1]{{/\!/\!_#1\,}} %reduced space



%Hyperref Package Additions

\newcommand{\hypref}[2]{{\hyperref[#1]{#2~\ref{#1}}}}


%Work Mode commands -- Work Mode (current version modified by me) was originally sent to me by Yael Karshon, but I forget who gave it to her.

\newcommand{\ifwork}[1]{\ifthenelse{\boolean{workmode}}{#1}{}}
\newcommand{\comment}[1]{}
\newcommand{\mute}[1]{}
\newcommand{\printname}[1]{}

\ifwork{
\renewcommand{\comment}[1]{{\marginpar{*}\ \scriptsize{#1}\ }}
%\renewcommand{\mute}[1]{{\scriptsize \ #1\ }\marginpar{\scriptsize muted}}
\renewcommand{\printname}[1]
    {\smash{\makebox[0pt]{\hspace{-1.0in}\raisebox{8pt}{\tiny #1}}}}
}

\newcommand{\labell}[1] {\label{#1} \printname{#1}}


%Theorem Styles

\newcommand{\ifsection}[2]{\ifthenelse{\boolean{sections}}{#1}{#2}}

\theoremstyle{plain}
\ifsection{
    \newtheorem{theorem}{Theorem}[section]
}
{
    \newtheorem{theorem}{Theorem}
}

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{question}[theorem]{Question}

% "End of Example" symbol

\def\eoe{\unskip\ \hglue0mm\hfill$\diamond$\smallskip\goodbreak} 
